MyStyle++: A Controllable Personalized Generative Prior

In this paper, we propose an approach to obtain a personalized generative prior with explicit control over a set of attributes. We build upon MyStyle, a recently introduced method, that tunes the weights of a pre-trained StyleGAN face generator on a few images of an individual. This system allows synthesizing, editing, and enhancing images of the target individual with high fidelity to their facial features. However, MyStyle does not demonstrate precise control over the attributes of the generated images. We propose to address this problem through a novel optimization system that organizes the latent space in addition to tuning the generator. Our key contribution is to formulate a loss that arranges the latent codes, corresponding to the input images, along a set of specific directions according to their attributes. We demonstrate that our approach, dubbed MyStyle++, is able to synthesize, edit, and enhance images of an individual with great control over the attributes, while preserving the unique facial characteristics of that individual.

==> 8_figures_sup.tex <==

% ----------------------------------------------------------------------------
\begin{figure}[hbt]
\centering
\includegraphics[width=1.0\linewidth, scale=1.0, angle=-0]{supp_images/image_synthesis_sampling_yawpitchexp_V4_bo.pdf}
% \vspace{-0.2in}
\caption{We present a comparison of our synthesis results with those of MyStyle\_I and MyStyle\_P on Barack Obama.}
\vspace{-0.1in}
\label{fig_sup:sampling_bo}
\end{figure}


% ----------------------------------------------------------------------------
% \begin{figure}
% \centering
% \includegraphics[width=1.0\linewidth, scale=1.0, angle=-0]{supp_images/image_synthesis_sampling_yawpitchexp_V4_jb.pdf}
% % \vspace{-0.2in}
% \caption{We present a comparison of our synthesis results with those of MyStyle\_I and MyStyle\_P on Joe Biden.}
% \vspace{-0.1in}
% \label{fig_sup:sampling_jb}
% \end{figure}

% ----------------------------------------------------------------------------
\begin{figure}
\centering
\includegraphics[width=1.0\linewidth, scale=1.0, angle=-0]{supp_images/image_synthesis_sampling_yawpitchexp_V4_mo.pdf}
% \vspace{-0.2in}
\caption{We present a comparison of our synthesis results with those of MyStyle\_I and MyStyle\_P on Michelle Obama.}
\vspace{-0.1in}
\label{fig_sup:sampling_mo}
\end{figure}

% ----------------------------------------------------------------------------
\begin{figure}
\centering
\includegraphics[width=1.0\linewidth, scale=1.0, angle=-0]{supp_images/image_synthesis_sampling_yawpitchexp_V4_ow.pdf}
% \vspace{-0.2in}
\caption{We present a comparison of our synthesis results with those of MyStyle\_I and MyStyle\_P on Oprah Winfrey.}
\vspace{-0.1in}
\label{fig_sup:sampling_ow}
\end{figure}

% ----------------------------------------------------------------------------
% \begin{figure}
% \centering
% \includegraphics[width=1.0\linewidth, scale=1.0, angle=-0]{supp_images/image_synthesis_sampling_yawpitchexp_V4_sj.pdf}
% % \vspace{-0.2in}
% \caption{We present a comparison of our synthesis results with those of MyStyle\_I and MyStyle\_P on Scarlett Johansson.}
% \vspace{-0.1in}
% \label{fig_sup:sampling_sj}
% \end{figure}

% ----------------------------------------------------------------------------
\begin{figure}
\centering
\includegraphics[width=1.0\linewidth, scale=1.0, angle=-0]{supp_images/image_synthesis_sampling_yawpitchexp_V4_ts.pdf}
% \vspace{-0.2in}
\caption{We present a comparison of our synthesis results with those of MyStyle\_I and MyStyle\_P on Taylor Swift.}
\vspace{-0.1in}
\label{fig_sup:sampling_ts}
\end{figure}

% ----------------------------------------------------------------------------
\begin{figure}
\centering
\includegraphics[width=1.0\linewidth, scale=1.0, angle=-0]{supp_images/image_synthesis_sampling_yawpitchexpage_V4_ew.pdf}
% \vspace{-0.2in}
\caption{We present a comparison of our synthesis results with those of MyStyle\_I and MyStyle\_P on Emma Watson.}
\vspace{-0.1in}
\label{fig_sup:sampling_ew}
\end{figure}

% ----------------------------------------------------------------------------
\begin{figure}
\centering
\includegraphics[width=1.0\linewidth, scale=1.0, angle=-0]{supp_images/image_synthesis_sampling_yawpitchexpage_V4_ld.pdf}
% \vspace{-0.2in}
\caption{We present a comparison of our synthesis results with those of MyStyle\_I and MyStyle\_P on Leonardo DiCaprio.}
\vspace{-0.1in}
\label{fig_sup:sampling_ld}
\end{figure}



% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------


% ----------------------------------------------------------------------------
\begin{figure}
\centering
\includegraphics[width=\linewidth, scale=1.0, angle=-0]{supp_images/image_editing_sampled_v6_bo.pdf}
% \vspace{-0.2in}
\caption{We show our results for editing expression, yaw, and pitch angles for sampled images against MyStyle\_P and MyStyle\_I on Barack Obama. Our method maintains the identity and consistency of other attributes while making modifications to the expression, yaw, or pitch of the image.}
% \vspace{-0.1in}
\label{fig_sup:editing_sampled_bo}
\end{figure}

% ----------------------------------------------------------------------------
\begin{figure}
\centering
\includegraphics[width=\linewidth, scale=1.0, angle=-0]{supp_images/image_editing_sampled_v6_jb.pdf}
% \vspace{-0.2in}
\caption{We show our results for editing expression, yaw, and pitch angles for sampled images against MyStyle\_P and MyStyle\_I on Joe Biden. Our method maintains the identity and consistency of other attributes while making modifications to the expression, yaw, or pitch of the image.}
% \vspace{-0.1in}
\label{fig_sup:editing_sampled_jb}
\end{figure}

% ----------------------------------------------------------------------------
% \begin{figure}
% \centering
% \includegraphics[width=\linewidth, scale=1.0, angle=-0]{supp_images/image_editing_sampled_v6_mo.pdf}
% % \vspace{-0.2in}
% \caption{We show our results for editing expression, yaw, and pitch angles for sampled images against MyStyle\_P and MyStyle\_I on Michelle Obama. Our method maintains the identity and consistency of other attributes while making modifications to the expression, yaw, or pitch of the image.}
% % \vspace{-0.1in}
% \label{fig_sup:editing_sampled_mo}
% \end{figure}

% ----------------------------------------------------------------------------
\begin{figure}
\centering
\includegraphics[width=\linewidth, scale=1.0, angle=-0]{supp_images/image_editing_sampled_v6_sj.pdf}
% \vspace{-0.2in}
\caption{We show our results for editing expression, yaw, and pitch angles for sampled images against MyStyle\_P and MyStyle\_I on Scarlett Johansson. Our method maintains the identity and consistency of other attributes while making modifications to the expression, yaw, or pitch of the image.}
% \vspace{-0.1in}
\label{fig_sup:editing_sampled_sj}
\end{figure}

% ----------------------------------------------------------------------------
% \begin{figure}
% \centering
% \includegraphics[width=\linewidth, scale=1.0, angle=-0]{supp_images/image_editing_sampled_age_V7_em.pdf}
% % \vspace{-0.2in}
% \caption{We show our results for editing expression, yaw, and pitch angles for sampled images against MyStyle\_P and MyStyle\_I on Emma Watson. Our method maintains the identity and consistency of other attributes while making modifications to the expression, yaw, or pitch of the image.}
% % \vspace{-0.1in}
% \label{fig_sup:editing_sampled_ew}
% \end{figure}

% ----------------------------------------------------------------------------
\begin{figure}
\centering
\includegraphics[width=\linewidth, scale=1.0, angle=-0]{supp_images/image_editing_sampled_age_V6_ld.pdf}
% \vspace{-0.2in}
\caption{We show our results for editing expression, yaw, pitch, and age for sampled images against MyStyle\_P and MyStyle\_I on Leonardo DiCaprio. Our method maintains the identity and consistency of other attributes while making modifications to the expression, yaw, pitch, or age of the image.}
% \vspace{-0.1in}
\label{fig_sup:editing_sampled_ld}
\end{figure}




% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------

% ----------------------------------------------------------------------------
\begin{figure*}
\centering
\includegraphics[width=\linewidth, scale=1.0, angle=-0]{supp_images/image_editing_sup_V12.pdf}
% \vspace{-0.2in}
\caption{We show comparisons against both versions of MyStyle for semantic editing of real images. Input is the projected images into the latent space of MyStyle and our generators. Our method disentangles the attributes better than MyStyle\_P and MyStyle\_I, producing results that preserve the unchanged attributes and identity. InterFaceGAN~\cite{shen2020interfacegan} does not provide an edit direction for pitch, and thus we leave the corresponding area of MyStyle\_I with a cross.
}
% \vspace{-0.1in}
\label{fig_sup:editing_real}
\end{figure*}


==> 9_tables_sup.tex <==

% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------

% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
\begin{table}[t] % not t or b or p
% \footnotesize
% \small
\caption{We numerically compare our controlled synthesis results against MyStyle\_P and MyStyle\_I. We generate 100 images for each fixed attribute value and report the standard deviation of the estimated attribute of interest over the generated images. Note that the attribute values (e.g., 0.25) are in the normalized coordinate $d_m$. The best results are shown in bold.}
%\vspace{-0.15in}
\centering
\begin{tabular}{ llccccc} 
% \begin{tabular*}{0.9\linewidth}{p{1.5cm} p{2.5cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm}}
\hline
\hline
& & \multicolumn{5}{c}{Barack Obama} \\
\cmidrule(lr){3-7}
& & 0.0 & 0.25 & 0.5 & 0.75 & 1.0 \\
\hline
\multirow{3}{*}{Exp} & MyStyle\_P & 0.664 & 0.822 & 0.846 & 0.915 & 0.899 \\
& MyStyle\_I& 0.855 & 0.866 & 0.894 & 0.740 & 0.701 \\
& Ours & \textbf{0.241} & \textbf{0.575} & \textbf{0.582} & \textbf{0.457} & \textbf{0.003} \\
\hline
\multirow{3}{*}{Yaw} & MyStyle\_P & 4.072 & 6.349 & 4.168 & 5.258 & 5.289 \\
& MyStyle\_I & 5.858 & 5.530 & 5.249 & 3.364 & 5.360 \\
& Ours & \textbf{1.951} & \textbf{1.952} & \textbf{1.846} & \textbf{2.158} & \textbf{1.900} \\
\hline
\multirow{3}{*}{Pitch} & MyStyle\_P & 5.748 & 4.061 & 7.127 & 6.295 & 5.611 \\
& MyStyle\_I & - & - & - & - & - \\
& Ours & \textbf{1.670} & \textbf{2.198} & \textbf{2.851} & \textbf{3.413} & \textbf{3.336} \\
% \hline  
\end{tabular}
% ----------------------------------------------------------------------------
\centering
\begin{tabular}{ llccccc} 
% \begin{tabular*}{0.9\linewidth}{p{1.5cm} p{2.5cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm}}
\hline
\hline
& & \multicolumn{5}{c}{Joe Biden} \\
\cmidrule(lr){3-7}
& & 0.0 & 0.25 & 0.5 & 0.75 & 1.0 \\
\hline
\multirow{3}{*}{Exp} & MyStyle\_P & 0.330 & 0.408 & 0.415 & 0.375 & 0.370 \\
& MyStyle\_I & 0.056 & 0.347 & 0.368 & 0.242 & 0.121 \\
& Ours & \textbf{0.031} & \textbf{0.216} & \textbf{0.329} & \textbf{221} & \textbf{0.013} \\
\hline
\multirow{3}{*}{Yaw} & MyStyle\_P & 6.725 & 6.411 & 5.071 & 9.103 & 7.652 \\
& MyStyle\_I & 5.578 & 3.777 & 3.474 & 4.832 & 6.687 \\
& Ours & \textbf{2.331} & \textbf{2.585} & \textbf{1.571} & \textbf{3.503} & \textbf{5.947} \\
\hline
\multirow{3}{*}{Pitch} & MyStyle\_P & 1.612 & 3.901 & 4.158 & 7.854 & 7.681 \\
& MyStyle\_I & - & - & - & - & - \\
& Ours & \textbf{4.061} & \textbf{3.669} & \textbf{1.431} & \textbf{2.464} & \textbf{2.117} \\
% \hline  
\end{tabular}
% ----------------------------------------------------------------------------
\centering
\begin{tabular}{ llccccc} 
% \begin{tabular*}{0.9\linewidth}{p{1.5cm} p{2.5cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm}}
\hline
\hline
& & \multicolumn{5}{c}{Michelle Obama} \\
\cmidrule(lr){3-7}
& & 0.0 & 0.25 & 0.5 & 0.75 & 1.0 \\
\hline
\multirow{3}{*}{Exp} & MyStyle\_P & 0.478 & 0.601 & 0.828 & 0.612 & 0.655 \\
& MyStyle\_I& 0.872 & 0.798 & 0.521 & 0.361 & 0.001 \\
& Ours & \textbf{0.169} & \textbf{0.378} & \textbf{0.217} & \textbf{0.038} & \textbf{0.000} \\
\hline
\multirow{3}{*}{Yaw} & MyStyle\_P & 3.239 & 4.464 & 2.757 & 5.195 & 4.835 \\
& MyStyle\_I & 4.473 & 2.920 & 3.692 & 4.077 & 4.523 \\
& Ours & \textbf{1.197} & \textbf{1.581} & \textbf{1.796} & \textbf{1.717} & \textbf{1.488} \\
\hline
\multirow{3}{*}{Pitch} & MyStyle\_P & 3.902 & 4.673 & 4.661 & 3.547 & 3.823 \\
& MyStyle\_I & - & - & - & - & - \\
& Ours & \textbf{2.426} & \textbf{2.264} & \textbf{1.699} & \textbf{1.823} & \textbf{1.687} \\
% \hline  
\end{tabular}
% ----------------------------------------------------------------------------
\centering
\begin{tabular}{ llccccc} 
% \begin{tabular*}{0.9\linewidth}{p{1.5cm} p{2.5cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm}}
\hline
\hline
& & \multicolumn{5}{c}{Oprah Winfrey} \\
\cmidrule(lr){3-7}
& & 0.0 & 0.25 & 0.5 & 0.75 & 1.0 \\
\hline
\multirow{3}{*}{Exp} & MyStyle\_P & 0.425 & 0.509 & 0.039 & 0.0024 & 0.006 \\
& MyStyle\_I& 0.067 & 0.371 & 0.003 & 0.009 & 0.002 \\
& Ours & \textbf{0.048} & \textbf{0.293} & \textbf{0.002} & \textbf{0.003} & \textbf{0.001} \\
\hline
\multirow{3}{*}{Yaw} & MyStyle\_P & 5.905 & 4.397 & 7.275 & 3.844 & 6.130 \\
& MyStyle\_I & 3.069 & 3.180 & 2.136 & 2.605 & 3.686 \\
& Ours & \textbf{1.333} & \textbf{2.704} & \textbf{1.649} & \textbf{1.532} & \textbf{1.119} \\
\hline
\multirow{3}{*}{Pitch} & MyStyle\_P & 4.551 & 4.470 & 3.765 & 3.788 & 4.181 \\
& MyStyle\_I & - & - & - & - & - \\
& Ours & \textbf{1.509} & \textbf{2.520} & \textbf{1.622} & \textbf{1.729} & \textbf{1.797} \\
\hline  
\end{tabular}

\label{sup_tab:syn_std_mean_1}
%\vspace{-0.2in}
\end{table}


% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
\begin{table}[t] % not t or b or p
% \footnotesize
% \small
\caption{We numerically compare our controlled synthesis results against MyStyle\_P and MyStyle\_I. We generate 100 images for each fixed attribute value and report the standard deviation of the estimated attribute of interest over the generated images. Note that the attribute values (e.g., 0.25) are in the normalized coordinate $d_m$. The best results are shown in bold.}
%\vspace{-0.15in}
\centering
\begin{tabular}{ llccccc} 
% \begin{tabular*}{0.9\linewidth}{p{1.5cm} p{2.5cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm}}
\hline
\hline
& & \multicolumn{5}{c}{Taylor Swift} \\
\cmidrule(lr){3-7}
& & 0.0 & 0.25 & 0.5 & 0.75 & 1.0 \\
\hline
\multirow{3}{*}{Exp} & MyStyle\_P & 0.673 & 0.612 & 0.582 & 0.611 & 300 \\
& MyStyle\_I& 0.361 & 0.602 & 0.355 & 0.690 & 0.677 \\
& Ours & \textbf{0.296} & \textbf{0.415} & \textbf{0.284} & \textbf{0.405} & \textbf{0.414} \\
\hline
\multirow{3}{*}{Yaw} & MyStyle\_P & 5.287 & 4.799 & 5.436 & 6.135 & 6.131 \\
& MyStyle\_I & 4.629 & 4.886 & 3.414 & 6.090 & 4.444 \\
& Ours & \textbf{1.618} & \textbf{2.187} & \textbf{2.843} & \textbf{2.443} & \textbf{1.657} \\
\hline
\multirow{3}{*}{Pitch} & MyStyle\_P & 5.012 & 5.005 & 2.566 & 3.089 & 4.156 \\
& MyStyle\_I & - & - & - & - & - \\
& Ours & \textbf{3.513} & \textbf{2.189} & \textbf{2.304} & \textbf{2.395} & \textbf{2.261} \\
% \hline  
\end{tabular}
% ----------------------------------------------------------------------------
\centering
\begin{tabular}{ llccccc} 
% \begin{tabular*}{0.9\linewidth}{p{1.5cm} p{2.5cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm}}
\hline
\hline
& & \multicolumn{5}{c}{Emma Watson}\\
\cmidrule(lr){3-7}
& & 0.0 & 0.25 & 0.5 & 0.75 & 1.0 \\
\hline
\multirow{3}{*}{Exp} & MyStyle\_P & 0.899 & 0.738 & 0.883 & 0.786 & 0.482 \\
& MyStyle\_I & 0.273 & 0.0.583 & 0.777 & 0.313 & 0.002 \\
& Ours & \textbf{0.005} & \textbf{0.004} & \textbf{0.531} & \textbf{0.213} & \textbf{0.001} \\
\hline
\multirow{3}{*}{Yaw} & MyStyle\_P & 4.353 & 5.834 & 5.156 & 4.268 & 3.948 \\
& MyStyle\_I & 3.277 & 3.146 & 1.997 & 3.133 & 3.080 \\
& Ours & \textbf{1.745} & \textbf{2.495} & \textbf{1.431} & \textbf{2.339} & \textbf{2.127} \\
\hline
\multirow{3}{*}{Pitch} & MyStyle\_P & 6.645 & 6.094 & 4.485 & 2.988 & 1.808 \\
& MyStyle\_I & - & - & - & - & -\\
& Ours & \textbf{4.887} & \textbf{2.714} & \textbf{1.758} & \textbf{2.374} & \textbf{1.426} \\
\hline
\multirow{3}{*}{Age} & MyStyle\_P & 2.760 & 2.016 & 0.899 & 1.041 & 1.062 \\
& MyStyle\_I & 3.775 & 2.502 & 0.873 & 1.171 & 1.920 \\
& Ours & \textbf{1.734} & \textbf{1.405} & \textbf{0.607} & \textbf{1.001} & \textbf{0.910} \\
\hline  
\end{tabular}
\label{sup_tab:syn_std_mean_2}
%\vspace{-0.2in}
\end{table}


% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------

% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
\begin{table}[t] % not t or b or p
% \footnotesize
% \small
\caption{We compare our results against MyStyle in terms of the ID metric~\cite{nitzan2022mystyle} and diversity score~\cite{ojha2021few}. Higher numbers are better. Our method produces similar results compared to MyStyles, which demonstrates that controllability does not hurt our system.}
\centering
\begin{tabular}{ >{\arraybackslash}m{0.7in} >{\arraybackslash}m{0.5in} >{\centering\arraybackslash}m{0.75in} >{\centering\arraybackslash}m{0.75in} }
% \begin{tabular}{ llc|c} 
% \begin{tabular*}{0.9\linewidth}{p{1.5cm} p{2.5cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm}}
\hline
\hline
& & \multicolumn{1}{c}{ID $\uparrow$ } & \multicolumn{1}{c}{Diversity $\uparrow$ }\\
% \cmidrule(lr){2-3}
% \cmidrule(lr){4-5}
\hline
\multirow{2}{*}{Barack Obama} & MyStyle & 0.787$\pm$0.053 & 0.393$\pm$0.070 \\
& Ours & 0.796$\pm$0.050 & 0.411$\pm$0.026 \\
\hline
\multirow{2}{*}{Emma Watson} & MyStyle & 0.734$\pm$0.090 & 0.453$\pm$0.023 \\
& Ours & 0.742$\pm$0.061 & 0.449$\pm$0.018 \\
\hline
\multirow{2}{*}{Joe Biden} & MyStyle & 0.759$\pm$0.004 & 0.397$\pm$0.023 \\
& Ours & 0.761$\pm$0.001 & 0.402$\pm$0.044 \\
\hline
\multirow{2}{*}{Michelle Obama} & MyStyle & 0.752$\pm$0.003  & 0.391$\pm$0.039 \\
& Ours & 0.757$\pm$0.004 & 0.389$\pm$0.024\\
\hline
\multirow{2}{*}{Oprah Winfrey} & MyStyle & 0.807$\pm$0.053 & 0.380$\pm$0.038 \\
& Ours & 0.821$\pm$0.058 & 0.380$\pm$0.057 \\
\hline
\multirow{2}{*}{Taylor Swift} & MyStyle & 0.775$\pm$0.065 & 0.393$\pm$0.049 \\
& Ours & 0.774$\pm$0.067 & 0.403$\pm$0.019 \\

\hline  
\end{tabular}
\label{tab_sup:syn_id_div}
\end{table}




% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------


% -----------------------moved--from--main------------------------------------
% ----------------------------------------------------------------------------
\begin{table}[htb] % not t or b or p
% \footnotesize
% \small
\caption{We compare our editing results against MyStyle\_I and MyStyle\_P in terms of the mean standard deviation (STD) of the edited attribute to show editing consistency (marked with $*$), and of fixed attributes to demonstrate attribute disentanglement. We additionally report the ID metric to evaluate identity preservation ability. The best results are shown in bold.}
\vspace{-0.15in}
\centering
\begin{tabular}{p{0.03\textwidth}>
{}p{0.07\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering\arraybackslash}p{0.1\textwidth}}
% \begin{tabular*}{0.9\linewidth}{p{1.5cm} p{2.5cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm}}
\hline
\hline
& & \multicolumn{4}{c}{Michelle Obama} \\
\cmidrule(lr){1-2}
\cmidrule(lr){3-6}
& & Exp$^{*}$ & Yaw & Pitch & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Exp} & MyStyle\_P  & 0.547 & 0.716 & 4.436 & 0.786$\pm$0.057\\
& MyStyle\_I  & 0.445 & 1.069 & 0.715 & 0.757$\pm$0.065 \\
& Ours & \textbf{0.306} & \textbf{0.576} & \textbf{0.596} & \textbf{0.794$\pm$0.034} \\

\hline
& & Yaw$^{*}$ & Exp & Pitch & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Yaw} & MyStyle\_P  & 2.773 & 0.477 & 2.419 & 0.780$\pm$0.053\\
& MyStyle\_I  & 4.424 & 0.510 & 2.181 & 0.715$\pm$0.110\\
& Ours  & \textbf{0.876} & \textbf{0.298} & \textbf{1.137} & \textbf{0.792$\pm$0.047} \\

\hline
& & Pitch$^{*}$ & Exp & Yaw & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Pitch} & MyStyle\_P  & 6.306 & 0.463 & 2.242 & 0.727$\pm$0.047\\
& MyStyle\_I & - & - & - & -\\
& Ours  & \textbf{2.045} & \textbf{0.231} & \textbf{1.311} & \textbf{0.731$\pm$0.110} \\
% \hline  
\end{tabular}

% ----------------------------------------------------------------------------
\centering
\begin{tabular}{p{0.03\textwidth}>
{}p{0.07\textwidth}>
{\centering}p{0.035\textwidth}>
{\centering}p{0.035\textwidth}>
{\centering}p{0.035\textwidth}>
{\centering}p{0.035\textwidth}>
{\centering\arraybackslash}p{0.1\textwidth}}
% \begin{tabular*}{0.9\linewidth}{p{1.5cm} p{2.5cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm}}
\hline
\hline
& & \multicolumn{5}{c}{Leonardo DiCaprio} \\
\cmidrule(lr){1-2}
\cmidrule(lr){3-7}
& & Exp$^{*}$ & Yaw & Pitch & Age & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-6}
\cmidrule(lr){7-7}
\multirow{3}{*}{Exp} & MyStyle\_P  & 0.794 & 4.866 & 1.965 & 3.584 & 0.743$\pm$0.103 \\
& MyStyle\_I  & 0.527 & 1.538 & 1.227 & 3.179 & 0.731$\pm$0.108 \\
& Ours & \textbf{0.268} & \textbf{1.204} & \textbf{0.999} & \textbf{2.201} & \textbf{0.752$\pm$0.107} \\
\hline
& & Yaw$^{*}$ & Exp & Pitch & Age & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-6}
\cmidrule(lr){7-7}
\multirow{3}{*}{Yaw} & MyStyle\_P  & 4.069 & 0.213 & 2.570 & 2.893 & 0.717$\pm$0.108 \\
& MyStyle\_I  & 3.925 & 0.111 & 2.426 & 2.700 & 0.716$\pm$0.117 \\
& Ours  & \textbf{2.097} & \textbf{0.075} & \textbf{2.108} & \textbf{2.212} & \textbf{0.728$\pm$0.115} \\

\hline
& & Pitch$^{*}$ & Exp & Yaw & Age & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-6}
\cmidrule(lr){7-7}
\multirow{3}{*}{Pitch} & MyStyle\_P  & 5.463 & 0.281 & 3.030 & 3.720 & 0.717$\pm$0.121 \\
& MyStyle\_I & - & - & - & - & - \\
& Ours  & \textbf{3.591} & \textbf{0.071} & \textbf{1.786} & \textbf{3.023} & \textbf{0.726$\pm$0.114} \\

\hline
& & Age$^{*}$ & Exp & Yaw & Pitch & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-6}
\cmidrule(lr){7-7}
\multirow{3}{*}{Age} & MyStyle\_P  & 5.113 & 0.230 & 2.808 & 2.824 & 0.734$\pm$0.118 \\
& MyStyle\_I & 7.152 & 0.134 & 1.294 & 2.095 & 0.723$\pm$0.120 \\
& Ours  & \textbf{3.473} & \textbf{0.087} & \textbf{0.467} & \textbf{1.217} & \textbf{0.739$\pm$0.113} \\
\hline  
\end{tabular}


\label{tab:edit_std}
\vspace{-0.15in}
\end{table}



% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
\begin{table}[t] % not t or b or p
% \footnotesize
% \small
\caption{We compare our editing results against MyStyle\_I and MyStyle\_P in terms of the mean standard deviation (STD) of edited attribute to show editing consistency (marked with $*$), and of fixed attributes to demonstrate attribute disentanglement. We additionally report the ID metric to evaluate identity preservation ability. The best results are shown in bold.}
%\vspace{-0.00in}
\centering
\begin{tabular}{p{0.03\textwidth}>
{}p{0.07\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering\arraybackslash}p{0.1\textwidth}}
% \begin{tabular*}{0.9\linewidth}{p{1.5cm} p{2.5cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm}}
\hline
\hline
& & \multicolumn{4}{c}{Barack Obama} \\
\cmidrule(lr){1-2}
\cmidrule(lr){3-6}
& & Exp$^{*}$ & Yaw & Pitch & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Exp} & MyStyle\_P  & 0.156 & 5.502 & 2.265 & 0.700$\pm$0.087\\
& MyStyle\_I  & 0.261 & 1.751 & 1.808 & 0.703$\pm$0.086\\
& Ours & \textbf{0.107} & \textbf{0.533} & \textbf{0.804} & \textbf{0.742$\pm$0.079} \\

\hline
& & Yaw$^{*}$ & Exp & Pitch & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Yaw} & MyStyle\_P  & 4.310 & 0.054 & 5.727 & 0.689$\pm$0.085\\
& MyStyle\_I  & 3.117 & 0.043 & 3.770 & 0.687$\pm$0.087\\
& Ours  & \textbf{1.524} & \textbf{0.028} & \textbf{2.349} & \textbf{0.709$\pm$0.083} \\

\hline
& & Pitch$^{*}$ & Exp & Yaw & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Pitch} & MyStyle\_P  & 5.131 & 0.031 & 6.285 & 0.692$\pm$0.087\\
& MyStyle\_I & - & - & - & -\\
& Ours  & \textbf{2.990} & \textbf{0.026} & \textbf{1.055} & \textbf{0.709$\pm$0.084} \\
% \hline  
\end{tabular}
% ----------------------------------------------------------------------------
\centering
\begin{tabular}{p{0.03\textwidth}>
{}p{0.07\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering\arraybackslash}p{0.1\textwidth}}
% \begin{tabular*}{0.9\linewidth}{p{1.5cm} p{2.5cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm}}
\hline
\hline
& & \multicolumn{4}{c}{Joe Biden} \\
\cmidrule(lr){1-2}
\cmidrule(lr){3-6}
& & Exp$^{*}$ & Yaw & Pitch & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Exp} & MyStyle\_P  & 0.776 & 1.809 & 5.619 & 0.654$\pm$0.091\\
& MyStyle\_I  & 0.446 & 1.707 & 1.054 & 0.693$\pm$0.072\\
& Ours & \textbf{0.332} & \textbf{1.095} & \textbf{1.254} & \textbf{0.703$\pm$0.076} \\
\hline
& & Yaw$^{*}$ & Exp & Pitch & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Yaw} & MyStyle\_P  & 10.42 & 0.739 & 10.50 & 0.666$\pm$0.084\\
& MyStyle\_I   & 9.190 & 0.789 & 2.341 & 0.676$\pm$0.077\\
& Ours  & \textbf{3.425} & \textbf{0.625} & \textbf{2.205} & \textbf{0.705$\pm$0.072} \\

\hline
& & Pitch$^{*}$ & Exp & Yaw & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Pitch} & MyStyle\_P   & 9.262 & 0.786 & 18.06 & 0.637$\pm$0.111\\
& MyStyle\_I & - & - & - & - \\
& Ours  & \textbf{3.958} & \textbf{0.603} & \textbf{2.656} & \textbf{0.693$\pm$0.080} \\
% \hline  
\end{tabular}
% ----------------------------------------------------------------------------
\centering
\begin{tabular}{p{0.03\textwidth}>
{}p{0.07\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering\arraybackslash}p{0.1\textwidth}}
% \begin{tabular*}{0.9\linewidth}{p{1.5cm} p{2.5cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm}}
\hline
\hline
& & \multicolumn{4}{c}{Oprah Winfrey} \\
\cmidrule(lr){1-2}
\cmidrule(lr){3-6}
& & Exp$^{*}$ & Yaw & Pitch & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Exp} & MyStyle\_P  & 0.303 & 4.358 & 3.335 & 0.685$\pm$0.100\\
& MyStyle\_I  & 0.140 & 1.738 & 1.523 & 0.690$\pm$0.092\\
& Ours & \textbf{0.116} & \textbf{0.531} & \textbf{0.401} & \textbf{0.712$\pm$0.088} \\
\hline
& & Yaw$^{*}$ & Exp & Pitch & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Yaw} & MyStyle\_P & 6.338 & 0.052 & 5.284 & 0.695$\pm$0.075\\
& MyStyle\_I  & 5.242 & 0.039 & 3.250 & 0.698$\pm$0.074\\
& Ours  & \textbf{2.330} & \textbf{0.027} & \textbf{2.425} & \textbf{0.702$\pm$0.075} \\

\hline
& & Pitch$^{*}$ & Exp & Yaw & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Pitch} & MyStyle\_P  & 4.949 & 0.053 & 3.423 & 0.657$\pm$0.104\\
& MyStyle\_I & - & - & - & - \\
& Ours  & \textbf{2.001} & \textbf{0.031} & \textbf{1.445} & \textbf{0.698$\pm$0.070} \\

\hline  
\end{tabular}

\label{tab_sup:edit_std_1}
%\vspace{-0.2in}
\end{table}








% ----------------------------------------------------------------------------
% ----------------------------------------------------------------------------
\begin{table}[htb] % not t or b or p
% \footnotesize
% \small
\caption{We compare our editing results against MyStyle\_I and MyStyle\_P in terms of the mean standard deviation (STD) of edited attribute to show editing consistency (marked with $*$), and of fixed attributes to demonstrate attribute disentanglement. We additionally report the ID metric to evaluate identity preservation ability. The best results are shown in bold.}
%\vspace{-0.00in}
\centering
\begin{tabular}{p{0.03\textwidth}>
{}p{0.07\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering\arraybackslash}p{0.1\textwidth}}
% \begin{tabular*}{0.9\linewidth}{p{1.5cm} p{2.5cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm}}
\hline
\hline
& & \multicolumn{4}{c}{Scarlett Johansson} \\
\cmidrule(lr){1-2}
\cmidrule(lr){3-6}
& & Exp$^{*}$ & Yaw & Pitch & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Exp} & MyStyle\_P  & 0.866 & 2.578 & 3.942 & 0.666$\pm$0.075\\
& MyStyle\_I  & 0.328 & 1.131 & 0.577 & 0.660$\pm$0.090\\
& Ours & \textbf{0.270} & \textbf{0.607} & \textbf{0.510} & \textbf{0.675$\pm$0.074} \\
\hline
& & Yaw$^{*}$ & Exp & Pitch & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Yaw} & MyStyle\_P & 9.216 & 0.869 & 1.671 & 0.686 $\pm$0.078\\
& MyStyle\_I   & 4.655 & 0.859 & 2.270 & 0.645$\pm$0.082\\
& Ours  & \textbf{2.349} & \textbf{0.774} & \textbf{1.669} & \textbf{0.707$\pm$0.069} \\

\hline
& & Pitch$^{*}$ & Exp & Yaw & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Pitch} & MyStyle\_P   & 5.639 & 0.924 & 5.755 & 0.667$\pm$0.077\\
& MyStyle\_I & - & - & - & - \\
& Ours  & \textbf{4.130} & \textbf{0.793} & \textbf{1.316} & \textbf{0.684$\pm$0.076} \\
% \hline  
\end{tabular}
% ----------------------------------------------------------------------------
\centering
\begin{tabular}{p{0.03\textwidth}>
{}p{0.07\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering}p{0.05\textwidth}>
{\centering\arraybackslash}p{0.1\textwidth}}
% \begin{tabular*}{0.9\linewidth}{p{1.5cm} p{2.5cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm}}
\hline
\hline
& & \multicolumn{4}{c}{Taylor Swift} \\
\cmidrule(lr){1-2}
\cmidrule(lr){3-6}
& & Exp$^{*}$ & Yaw & Pitch & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Exp} & MyStyle\_P  & 0.783 & 3.421 & 3.933 & 0.698$\pm$0.077\\
& MyStyle\_I  & 0.314 & 2.444 & 1.237 & 0.683$\pm$0.079\\
& Ours & \textbf{0.230} & \textbf{1.532} & \textbf{0.783} & \textbf{0.713$\pm$0.077} \\
\hline
& & Yaw$^{*}$ & Exp & Pitch & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Yaw} & MyStyle\_P  & 7.343 & 0.783 & 3.210 & 0.688$\pm$0.087\\
& MyStyle\_I   & 3.598 & 0.389 & 2.333 & 0.700$\pm$0.074\\
& Ours  & \textbf{1.925} & \textbf{0.241} & \textbf{1.982} & \textbf{0.720$\pm$0.069} \\

\hline
& & Pitch$^{*}$ & Exp & Yaw & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-6}
\multirow{3}{*}{Pitch} & MyStyle\_P   & 4.189 & 0.102 & 5.283 & 0.703$\pm$0.078\\
& MyStyle\_I & - & - & - & - \\
& Ours  & \textbf{2.374} & \textbf{0.041} & \textbf{2.338} & \textbf{0.721$\pm$0.079} \\
% \hline  
\end{tabular}
% ----------------------------------------------------------------------------
\centering
\begin{tabular}{p{0.03\textwidth}>
{}p{0.07\textwidth}>
{\centering}p{0.035\textwidth}>
{\centering}p{0.035\textwidth}>
{\centering}p{0.035\textwidth}>
{\centering}p{0.035\textwidth}>
{\centering\arraybackslash}p{0.1\textwidth}}
% \begin{tabular*}{0.9\linewidth}{p{1.5cm} p{2.5cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm} p{2.0cm}}
\hline
\hline
& & \multicolumn{5}{c}{Emma Watson} \\
\cmidrule(lr){1-2}
\cmidrule(lr){3-7}
& & Exp$^{*}$ & Yaw & Pitch & Age & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-6}
\cmidrule(lr){7-7}
\multirow{3}{*}{Exp} & MyStyle\_P  & 0.821  & 3.892 & 2.721 & 4.021 & 0.698$\pm$0.113\\
& MyStyle\_I   & 0.482  & 1.732 & 2.034 & 3.248 & 0.710$\pm$0.096\\
& Ours & \textbf{0.240} & \textbf{1.330} & \textbf{1.218} & \textbf{2.017} & \textbf{0.748$\pm$0.094} \\
\hline
& & Yaw$^{*}$ & Exp & Pitch & Age & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-6}
\cmidrule(lr){7-7}
\multirow{3}{*}{Yaw} & MyStyle\_P   & 5.478  & 0.432 & 3.258 & 3.483 & 0.728$\pm$0.090\\
& MyStyle\_I  & 4.130  & 0.384& 2.832 & 3.003 & 0.713$\pm$0.094\\
& Ours  & \textbf{2.783} & \textbf{0.104} & \textbf{2.203} & \textbf{2.438} & \textbf{0.733$\pm$0.092} \\

\hline
& & Pitch$^{*}$ & Exp & Yaw & Age & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-6}
\cmidrule(lr){7-7}
\multirow{3}{*}{Pitch} & MyStyle\_P   & 4.389  & 0.492 & 3.189 & 3.899 & 0.728$\pm$0.096\\
& MyStyle\_I & - & - & - & - & -\\
& Ours  & \textbf{3.294} & \textbf{0.085} & \textbf{1.839} & \textbf{2.893} & \textbf{0.746$\pm$0.094} \\

\hline
& & Age$^{*}$ & Exp & Yaw & Pitch & ID $\uparrow$\\
\cmidrule(lr){3-3}
\cmidrule(lr){4-6}
\cmidrule(lr){7-7}
\multirow{3}{*}{Age} & MyStyle\_P   & 4.883  & 0.432 & 3.543 & 2.983 & 0.717$\pm$0.086\\
& MyStyle\_I  & 4.238  & 0.233 & 2.899 & 2.339 & 0.725$\pm$0.114\\
& Ours  & \textbf{2.938} & \textbf{0.183} & \textbf{1.032} & \textbf{1.384} & \textbf{0.742$\pm$0.082} \\
\hline  
\end{tabular}

\label{tab_sup:edit_std_2}
%\vspace{-0.2in}
\end{table}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
